TESTQUEST: A Web Gamification Tool to Improve Locators and Page Objects Quality

Web applications play a crucial role in our daily lives, making it essential to employ testing methods that ensure their quality. Typically, Web testing automation frameworks rely on locators to interact with the graphical user interface, acting as connection points to the elements on a Web page. Nevertheless, locators are widely recognized as a major vulnerability in Web testing, as they are highly sensitive to the frequent changes in Web page structures caused by rapid software evolution. The adoption of the Page Object pattern to separate test logic from structural layout - supporting code reuse and maintainability - has generally led to more robust test cases. However, their implementation is a manually intensive task, and even automated support may require manual realignment efforts. Although gamification strategies have recently been integrated into the Web testing process to boost user engagement, using tasks and rewards aligned with testing activities, they have not yet been employed to enhance the robustness of locators and support the implementation of Page Objects. In this paper, we introduce TESTQUEST, a tool designed to improve test robustness by applying gamification to locators and Page Objects, boosting user engagement while guiding them toward the adoption of best practices.

==> 40-testSuites.tex <==
tbd

==> 60-related.tex <==
tbd
